Polygonal approximations of closed parametric varifolds

We define holonomic measures to be certain analogues of varifolds that keep track of the local parameterization and orientation of the submanifold they represent. They are Borel measures on the direct sum of several copies of the tangent bundle. We show that there is an approximation to these by smooth singular chains whose boundaries and Lagrangian actions are controlled. As an illustration of the usefulness of this result, we show how this can be applied to study foliations on the torus. We give other applications elsewhere.

==> density.tex <==
For each set  $C=\{V_1\supset\cdots\supset V_{n-1}\}\subset T_k$ of properly nested simplices, in Section \ref{sec:cyclesconstruction} the 1-dimensional chain $\finalchain^C$ was constructed. Our goal in this section is to estimate the asymptotic behavior of its mass $\mass(\measure{\finalchain^C})$ as $k\to\infty$.

For a set $U\subset\R^m$, the \emph{diameter of $U$ within $U$} is defined to be
\[\diam_UU=\sup_{x,y\in U}\inf_\gamma \arclength(\gamma)\]
where the infimum is taken over all absolutely-continuous curves $\gamma$ parameterized on all intervals $[a,b]\subseteq\R$ and such that $\gamma(a)=x$ and $\gamma(b)=y$.

\begin{lem}\label{lem:density}
Let $U$ be a path-connected, bounded open set in $\R^m$, $m\geq 1$.
There is a number $\varepsilon_0>0$ such that if $0<\varepsilon<\varepsilon_0$ and $A$ and $B$ are two finite subsets of $U$
of equal cardinality, then the following is true. Assume that there is a finite partition of $U$ by disjoint, path-connected sets $U_1,\dots,U_m$ with $\diam_{U_i} U_i<\varepsilon$
such that each of them contains at least one point of $A$, and
\begin{equation}\label{eq:densitycondition}
\left|1-\frac{\#U_i\cap B}{\#U_i\cap A}\right|<\varepsilon^2.
\end{equation}
Then there is a 1-dimensional chain $\theta$ such that $\measure\theta(U)=1$, $\mass\left(\measure\theta\right)<2\varepsilon$, and 
\begin{equation}\label{eq:smallconnections}
\partial\theta=\frac{1}{\#A}\left(\sum_{x\in A}x-\sum_{y\in B}y\right).
\end{equation}
\end{lem}
\begin{rmk}
Equation \eqref{eq:smallconnections} should be interpreted in the sense of boundaries of singular homology (cf. \cite[\S2.1]{hatcher}).
\end{rmk}
\begin{proof}
Let 
\[\varepsilon_0=\frac{1}{2\diam_UU}.\]
Condition \eqref{eq:densitycondition} implies that at least $\lfloor(1-\varepsilon^2)\#U_i\cap A\rfloor$ points of $A$ can be joined to points of $B$ within $U_i$. Since $\diam_{U_i}U_i<\varepsilon$, this can be done using curves $\gamma$ of length smaller than $\varepsilon$. Let $\lambda_1$ be the chain formed by all those curves $\gamma$, each parameterized at the right speed that its induced measure will be a probability, $\measure\gamma(TU)=1$. The remaining $\sim\varepsilon^2\#U_i\cap A$ points of $A$ (and a similar amount of points of $B$) need to be paired with points outside $U_i$. Since $\#A=\#B$, this is always possible, and it can be done using curves of length $\leq \diam_UU$. Let $\lambda_2$ be the chain corresponding to these longer curves, again parameterized at a speed that will make the induced measure a probability. 

We let $\theta=(\lambda_1+\lambda_2)/\#A$. It is clear then that $\measure\theta$ is a probability, and that \eqref{eq:smallconnections} holds. We estimate
\begin{multline*}
\mass\left(\measure\theta\right) =\frac{\arclength(\lambda_1)+\arclength(\lambda_2)}{\#A}\\ \leq\frac{\varepsilon(1-\varepsilon^2)\#A+(\diam_UU)\varepsilon^2\#A}{\#A}\leq 2\varepsilon.\qedhere
\end{multline*}
\end{proof}

Let $k\geq 1$ and let $C$ be a set of properly nested simplices in $T_k$. Decompose the chain $\finalchain^{C}$ into the part of it that comes from $\bar\baseapprox_k^{C}$ and a remainder $\remainder^C_k$,
\[\finalchain^{C}=\bar\baseapprox_k^{C}+\remainder^{C}_k.\]

Fix $k\in\N$ and a set $C$ of $n$ properly nested simplices. 
From the construction of $\finalchain^C$, it follows that $\remainder^C_k$ is formed from two types of components:
\begin{itemize}
 \item Curves joining two points in the 0-chains
 %\footnote{The reader is reminded that $\baseapprox^C_k$ lives in the boundary of the simplex in which $\bar\baseapprox^C_k$ lives.} 
 $\baseapprox^{C}_k$; call the corresponding chain $\zetashort$.
 \item Curves joining points in various 0-chains $\finalchain^{C'}$ ($C'\supset C$) that are not both already in $\baseapprox^{C}_k$; call the corresponding chain $\zetalong$.
\end{itemize}

Observe that as $k\to\infty$, the first quotient in \eqref{eq:densityofsample} behaves as
\[\frac{\base_k(V_2)}{\base_k(V_1)}\to1\]
since the triangulations $T_k$ satisfy T\ref{it:vanishingdiameter} and $\mu$ is assumed to be a smooth density. So \eqref{eq:densityofsample} tends to look like \eqref{eq:densitycondition}.  It follows that if $k$ is large, we can apply Lemma \ref{lem:density} to a large subset of the points of $\partial\zetashort$, with the conclusion that the part of $\zetashort$ joining them has very small mass $\mass$. What remains of $\partial\zetashort$ tends to have 0 weight, so the mass of the corresponding part of $\zetashort$ also vanishes asymptotically. 

Similarly, since $\base_k\to\mu$ as $k\to\infty$, and since the points $\{p_i^k\}_i$ are a sample of $\mu|_{E^k_{d-n}}$ (they satisfy U\ref{U:isofrightmass}), the weight of $\partial\zetalong$ vanishes asymptotically, and hence so does the mass of $\zetalong$.

We let the function $a$ in A\ref{it:densityassumption} decrease rapidly enough that the following lemma will hold as per the preceding argument.
\begin{lem}\label{lem:onechains}
As $k\to\infty$,
\[\sum_C\mass(\measure{\remainder^C_k})\to 0\qquad\textrm{and}\qquad \frac{\sum_C\mass(\measure{\finalchain^C})}{\sum_C \mass(\measure{\bar\baseapprox_k^C})} \to 1, \]
where the sums are taken over all sets $C$ of $n-1$ properly nested simplices in $T_k$. 
\end{lem}







